The canonical ring of a stacky curve

Generalizing the classical theorems of Max Noether and Petri, we describe generators and relations for the canonical ring of a stacky curve, including an explicit Gr\"obner basis. We work in a general algebro-geometric context and treat log canonical and spin canonical rings as well. As an application, we give an explicit presentation for graded rings of modular forms arising from finite-area quotients of the upper half-plane by Fuchsian groups.

==> frontmatter/bigHeader.tex <==
\usepackage{pdfsync}
\usepackage{amssymb}
\usepackage{stmaryrd}
\usepackage{fullpage}	% smaller margins
\usepackage{amscd}   	% for commutative diagrams
\usepackage[all]{xy}       % for complicated commutative diagrams
\usepackage{comment} 	% for \begin{comment} ... \end{comment}
\usepackage{mathrsfs}   % for \mathscr
% Note: if you have problems with the Sha in cyrillic font,
% change the following ``paragraph'' to \newcommand{\Sha}{{\operatorname{Sha}}}
\usepackage{array}         % allows me to fix vertical spacing


\DeclareFontEncoding{OT2}{}{} % to enable usage of cyrillic fonts
\newcommand{\textcyr}[1]{%
 {\fontencoding{OT2}\fontfamily{wncyr}\fontseries{m}\fontshape{n}\selectfont #1}}
\newcommand{\Sha}{{\mbox{\textcyr{Sh}}}}
% note: cmr might work in place of wncyr

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% for cartesian diagrams
 \newcommand{\pb}{\rule{.4pt}{5.4pt}\rule[5pt]{5pt}{.4pt}\llap{$\cdot$\hspace{1pt}}}


\newcommand{\PROJ}{{\mathbb Proj}}


\newcommand{\defi}[1]{\textsf{#1}} 				% for defined terms


\newcommand{\known}{{\operatorname{known}}}
\newcommand{\Abar}{{\overline{A}}}
\newcommand{\To}{\longrightarrow}
\newcommand{\nichts}{\ensuremath{\left.\right.}}
\newcommand{\ssigma}{{\! \nichts^\sigma \!}
}
\newcommand{\GQp}{{{\mathcal G}_{\Q_p}}}
\newcommand{\Gk}{{{\mathcal G}_k}}
\newcommand{\GK}{{{\mathcal G}_K}}
%\newcommand{\YY}{{\mathcal Y}}
\newcommand{\prim}{{\operatorname{prim}}}
\newcommand{\fake}{{\operatorname{fake}}}
\newcommand{\conts}{{\operatorname{conts}}}
\newcommand{\wedgeisom}{{\;\stackrel{\wedge}\isom}\;}
\newcommand{\xbar}{{\bar{x}}}
\newcommand{\ybar}{{\bar{y}}}
\newcommand{\zbar}{{\bar{z}}}
\newcommand{\Xtilde}{{\tilde{X}}}
\newcommand{\pitilde}{{\tilde{\pi}}}
\newcommand{\subs}{{\operatorname{subset}}}
\newcommand{\umtp}[1]{#1^\times\!/(#1^\times)^3}


% Characters
\newcommand{\Aff}{{\mathbb A}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\G}{{\mathbb G}}
\newcommand{\bbH}{{\mathbb H}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Qbar}{{\overline{\Q}}}
\newcommand{\Zhat}{{\hat{\Z}}}
\newcommand{\Zbar}{{\overline{\Z}}}
\newcommand{\kbar}{{\overline{k}}}
\newcommand{\Kbar}{{\overline{K}}}
\newcommand{\ksep}{{k^{\operatorname{sep}}}}
\newcommand{\Fbar}{{\overline{\F}}}

\newcommand{\Adeles}{{\mathbf A}}
\newcommand{\kk}{{\mathbf k}}

\newcommand{\pp}{{\mathfrak p}}
\newcommand{\frakq}{{\mathfrak q}}
\newcommand{\qq}{{\mathfrak q}}
\newcommand{\mm}{{\mathfrak m}}



% mathcal characters
\newcommand{\calA}{{\mathcal A}}
\newcommand{\calB}{{\mathcal B}}
\newcommand{\calC}{{\mathcal C}}
\newcommand{\calD}{{\mathcal D}}
\newcommand{\calE}{{\mathcal E}}
\newcommand{\calF}{{\mathcal F}}
\newcommand{\calG}{{\mathcal G}}
\newcommand{\calH}{{\mathcal H}}
\newcommand{\calI}{{\mathcal I}}
\newcommand{\calJ}{{\mathcal J}}
\newcommand{\calK}{{\mathcal K}}
\newcommand{\calL}{{\mathcal L}}
\newcommand{\calM}{{\mathcal M}}
\newcommand{\calN}{{\mathcal N}}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calP}{{\mathcal P}}
\newcommand{\calQ}{{\mathcal Q}}
\newcommand{\calR}{{\mathcal R}}
\newcommand{\calS}{{\mathcal S}}
\newcommand{\calT}{{\mathcal T}}
\newcommand{\calU}{{\mathcal U}}
\newcommand{\calV}{{\mathcal V}}
\newcommand{\calW}{{\mathcal W}}
\newcommand{\calX}{{\mathcal X}}
\newcommand{\calY}{{\mathcal Y}}
\newcommand{\calZ}{{\mathcal Z}}
\newcommand{\FF}{{\mathcal F}}
\newcommand{\GG}{{\mathcal G}}
\newcommand{\II}{{\mathcal I}}
\newcommand{\JJ}{{\mathcal J}}
\newcommand{\LL}{{\mathcal L}}
\newcommand{\OO}{{\mathcal O}}

% mathscr characters
\newcommand{\scrA}{{\mathscr A}}
\newcommand{\scrB}{{\mathscr B}}
\newcommand{\scrC}{{\mathscr C}}
\newcommand{\scrD}{{\mathscr D}}
\newcommand{\scrE}{{\mathscr E}}
\newcommand{\scrF}{{\mathscr F}}
\newcommand{\scrG}{{\mathscr G}}
\newcommand{\scrH}{{\mathscr H}}
\newcommand{\scrI}{{\mathscr I}}
\newcommand{\scrJ}{{\mathscr J}}
\newcommand{\scrK}{{\mathscr K}}
\newcommand{\scrL}{{\mathscr L}}
\newcommand{\scrM}{{\mathscr M}}
\newcommand{\scrN}{{\mathscr N}}
\newcommand{\scrO}{{\mathscr O}}
\newcommand{\scrP}{{\mathscr P}}
\newcommand{\scrQ}{{\mathscr Q}}
\newcommand{\scrR}{{\mathscr R}}
\newcommand{\scrS}{{\mathscr S}}
\newcommand{\scrT}{{\mathscr T}}
\newcommand{\scrU}{{\mathscr U}}
\newcommand{\scrV}{{\mathscr V}}
\newcommand{\scrW}{{\mathscr W}}
\newcommand{\scrX}{{\mathscr X}}
\newcommand{\scrY}{{\mathscr Y}}
\newcommand{\scrZ}{{\mathscr Z}}

\def\Q{\mathbb{Q}}
\def\C{\mathbb{C}}
\def\R{\mathbb{R}}
\def\P{\mathbb{P}}
\def\A{\mathbb{A}}
\def\Z{\mathbb{Z}}

\def\Qb{\bar{\mathbb{Q}}}
\def\kb{\bar{k}}

\def\hb{\hat{h}}


% Math operators
%\DeclareMathOperator{\th}{th}
\DeclareMathOperator{\tr}{tr} \DeclareMathOperator{\trdeg}{tr deg}
\DeclareMathOperator{\coker}{coker} \DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\Char}{char} \DeclareMathOperator{\inv}{inv}
\DeclareMathOperator{\nil}{Nil} \DeclareMathOperator{\im}{im}
\DeclareMathOperator{\re}{Re} \DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Jac}{Jac} \DeclareMathOperator{\END}{\bf End}
\DeclareMathOperator{\Lie}{Lie} \DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\HOM}{\bf Hom} \DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Gal}{Gal} \DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\Cor}{Cor} \DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Norm}{Norm} \DeclareMathOperator{\Br}{Br}
\DeclareMathOperator{\Gr}{Gr} \DeclareMathOperator{\cd}{cd}
\DeclareMathOperator{\scd}{scd} \DeclareMathOperator{\Sel}{Sel}
\DeclareMathOperator{\Cl}{Cl} \DeclareMathOperator{\divv}{div}
\DeclareMathOperator{\ord}{ord} \DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Div}{Div} \DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Num}{Num} \DeclareMathOperator{\PIC}{\bf Pic}
\DeclareMathOperator{\Spec}{Spec} \DeclareMathOperator{\SPEC}{\bf Spec} 
\DeclareMathOperator{\Proj}{Proj} 
\DeclareMathOperator{\Frac}{Frac} \DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\CaCl}{CaCl}
\DeclareMathOperator{\Mod}{Mod}
\DeclareMathOperator{\Open}{Open}
\DeclareMathOperator{\Coh}{Coh}
\DeclareMathOperator{\id}{id}





% Categories
\newcommand{\Schemes}{\operatorname{\bf Schemes}}
\newcommand{\Sch}{\operatorname{\bf Sch}}
\newcommand{\Sets}{\operatorname{\bf Sets}}
%\newcommand{\Ab}{\operatorname{\bf Ab}}
\newcommand{\Ab}{\operatorname{Ab}}
\newcommand{\Groups}{\operatorname{\bf Groups}}

% Text subscripts, superscripts
\newcommand{\perf}{{\operatorname{perf}}}
\newcommand{\op}{{\operatorname{op}}}
\newcommand{\an}{{\operatorname{an}}}
\newcommand{\ab}{{\operatorname{ab}}}
\newcommand{\smooth}{{\operatorname{smooth}}}
\newcommand{\sing}{{\operatorname{sing}}}
\newcommand{\CS}{\operatorname{\bf CS}}
\newcommand{\Zar}{{\operatorname{Zar}}}
\newcommand{\fl}{{\operatorname{f\textcompwordmark l}}}
\newcommand{\et}{{\operatorname{et}}}
\newcommand{\Az}{{\operatorname{Az}}}
\newcommand{\ET}{{\operatorname{\bf \acute{E}t}}}
\newcommand{\tors}{{\operatorname{tors}}}
\newcommand{\red}{{\operatorname{red}}}
\newcommand{\unr}{{\operatorname{unr}}}
\newcommand{\tH}{{\operatorname{th}}}


\newcommand{\GalQ}{{\Gal}(\Qbar/\Q)}
\newcommand{\Cech}{\v{C}ech\xspace}
\newcommand{\HH}{{\operatorname{H}}}
\newcommand{\HHcech}{{\check{\HH}}}
\newcommand{\HHat}{{\hat{\HH}}}
\newcommand{\M}{\operatorname{M}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\PSL}{\operatorname{PSL}}

\newcommand{\surjects}{\twoheadrightarrow}
\newcommand{\injects}{\hookrightarrow}
\newcommand{\isom}{\simeq}
\newcommand{\notdiv}{\nmid}
\newcommand{\del}{\partial}
\newcommand{\Intersection}{\bigcap}
\newcommand{\intersect}{\cap}
\newcommand{\Union}{\bigcup}
\newcommand{\union}{\cup}
\newcommand{\tensor}{\otimes}
\newcommand{\directsum}{\oplus}
\newcommand{\Directsum}{\bigoplus}

\newcommand{\isomto}{\overset{\sim}{\rightarrow}}
\newcommand{\isomfrom}{\overset{\sim}{\leftarrow}}
\newcommand{\leftexp}[2]{{\vphantom{#2}}^{#1}{#2}}
\newcommand{\sigmaiota}{{\leftexp{\sigma}{\iota}}}
\newcommand{\sigmaphi}{{\leftexp{\sigma}{\phi}}}
\newcommand{\tauphi}{{\leftexp{\tau}{\phi}}}
\newcommand{\sigmatauphi}{{\leftexp{\sigma\tau}{\phi}}}


%%% Uncomment these to number equations by section
\numberwithin{equation}{subsection}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{proposition}[equation]{Proposition}

\theoremstyle{definition}
\newtheorem{definition}[equation]{Definition}
\newtheorem{question}[equation]{Question}
\newtheorem{answer}[equation]{Answer}
\newtheorem{fact}[equation]{Fact}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{example}[equation]{Example}

\theoremstyle{remark}
\newtheorem{remark}[equation]{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{warning}[equation]{Warning}
%% Ending here.


%%% Uncomment these to have unnumbered equations
%\newtheorem*{theorem}{Theorem}
%\newtheorem*{lemma}{Lemma}
%\newtheorem*{corollary}{Corollary}
%\newtheorem*{proposition}{Proposition}
%
%\theoremstyle{definition}
%\newtheorem*{definition}{Definition}
%\newtheorem*{question}{Question}
%\newtheorem*{conjecture}{Conjecture}
%\newtheorem*{example}{Example}
%
%\theoremstyle{remark}
%\newtheorem*{remark}{Remark}
%\newtheorem*{remarks}{Remarks}
%\newtheorem*{warning}{Warning}
%%% Ending here.

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{question}[theorem]{Question}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{example}[theorem]{Example}
%
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{remarks}[theorem]{Remarks}
%\newtheorem{warning}[theorem]{Warning}


\input{extraHeader.tex}

\renewcommand{\arraystretch}{1.4}
\renewcommand{\baselinestretch}{1.1}   % for spacing

%\newcommand{\marg}[1]{\marginpar{\small #1}}
% \newcommand{\marg}[1]{(*)\marginpar{\small #1}}
 \newcommand{\marg}[1]{}

\usepackage[
%	draft,
%	colorlinks,
	backref,
	pdfauthor={David Brown}, % add other authors
%	pdftitle={Paper title goes here},
]{hyperref}

\usepackage[alphabetic,backrefs,lite]{amsrefs} % for bibliography

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../stacky-canonical-rings"
%%% End: 


==> frontmatter/packages.tex <==

\usepackage{wasysym}
\usepackage{url}
\usepackage{hyperref}
\usepackage{pdfsync}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{stmaryrd}
\usepackage{fullpage}	% smaller margins %incompatible with ucthesis
\usepackage{amscd}   	% for commutative diagrams
\usepackage[all]{xy} 		% for complicated commutative diagrams
\usepackage{comment} 	% for \begin{comment} ... \end{comment}
\usepackage{mathrsfs}      % for \mathscr


\usepackage[style=alphabetic]{biblatex}
\usepackage{filecontents}





\usepackage{tikz}
%\usepackage{picinpar} % for pictures in paragraphs
\usetikzlibrary{decorations.pathmorphing}


\usepackage{enumerate}

\usepackage{tikz}
%\usepackage{picinpar} % for pictures in paragraphs
\usetikzlibrary{decorations.pathmorphing}




\usepackage[alphabetic,backrefs,lite,bibtex-style]{amsrefs} % for bibliography



%%%%%%%%%%%%%% COLOR COMMENTS! %%%%%%%%%%%%%%%
\usepackage{color}
\newcommand{\aaron}[1]{{\color{red} \sf    $\spadesuit\spadesuit\spadesuit$ Comment from Aaron: [#1]}}
\newcommand{\david}[1]{{\color{blue} \sf $\spadesuit\spadesuit\spadesuit$ David: [#1]}}
\newcommand{\alsodavid}[1]{{\color{green} \sf    $\spadesuit\spadesuit\spadesuit$ Also David: [#1]}}
\newcommand{\jv}[1]{{\color{red} \sf $\clubsuit\clubsuit\clubsuit$ JV: [#1]}}
\newcommand{\details}[1]{{\color{brown} \sf #1 }}


% changed above definition to make comments disappear
% \newcommand{\aaron}[1]{}
%\newcommand{\david}[1]{}
%\newcommand{\alsodavid}[1]{}
%\newcommand{\bjorn}[1]{}
%\newcommand{\details}[1]{}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../stacky-canonical-rings"
%%% End: 


==> frontmatter/theoremStyle.tex <==
%%% Uncomment these to number equations by equation
\numberwithin{equation}{subsection}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{proposition}[equation]{Proposition}

\theoremstyle{definition}
\newtheorem{definition}[equation]{Definition}
\newtheorem{question}[equation]{Question}
\newtheorem{answer}[equation]{Answer}
\newtheorem{fact}[equation]{Fact}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{example}[equation]{Example}
%\newtheorem{para}[equation]{}

\theoremstyle{remark}
\newtheorem{remark}[equation]{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{warning}[equation]{Warning}
\newtheorem*{claim}{Claim}

\newcommand{\labelpar}[1]{\refstepcounter{equation}\label{#1}\theequation.}
%% Ending here.



% %%% Uncomment these to number equations by equation
% \numberwithin{equation}{equation}
% \newtheorem{theorem}[equation]{Theorem}
% \newtheorem{lemma}[equation]{Lemma}
% \newtheorem{corollary}[equation]{Corollary}
% \newtheorem{proposition}[equation]{Proposition}

% \theoremstyle{definition}
% \newtheorem{definition}[equation]{Definition}
% \newtheorem{question}[equation]{Question}
% \newtheorem{answer}[equation]{Answer}
% \newtheorem{fact}[equation]{Fact}
% \newtheorem{conjecture}[equation]{Conjecture}
% \newtheorem{example}[equation]{Example}
% \newtheorem{para}[equation]{}

% \theoremstyle{remark}
% \newtheorem{remark}[equation]{Remark}
% \newtheorem{remarks}[equation]{Remarks}
% \newtheorem{warning}[equation]{Warning}
%\newcommand{\labelpar}[1]{\refstepcounter{equation}\label{#1}\theequation.}
% %% Ending here.


%%% Uncomment these to have unnumbered equations
%\newtheorem*{theorem}{Theorem}
%\newtheorem*{lemma}{Lemma}
%\newtheorem*{corollary}{Corollary}
%\newtheorem*{proposition}{Proposition}
%
%\theoremstyle{definition}
%\newtheorem*{definition}{Definition}
%\newtheorem*{question}{Question}
%\newtheorem*{conjecture}{Conjecture}
%\newtheorem*{example}{Example}
%
%\theoremstyle{remark}
%\newtheorem*{remark}{Remark}
%\newtheorem*{remarks}{Remarks}
%\newtheorem*{warning}{Warning}
%%% Ending here.

%\newtheorem{theorem}{Theorem}[equation]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{question}[theorem]{Question}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{example}[theorem]{Example}
%
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{remarks}[theorem]{Remarks}
%\newtheorem{warning}[theorem]{Warning}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../stacky-canonical-rings"
%%% End: 

